CLASSIC: Continual and Contrastive Learning of Aspect Sentiment Classification Tasks

This paper studies continual learning (CL) of a sequence of aspect sentiment classification(ASC) tasks in a particular CL setting called domain incremental learning (DIL). Each task is from a different domain or product. The DIL setting is particularly suited to ASC because in testing the system needs not know the task/domain to which the test data belongs. To our knowledge, this setting has not been studied before for ASC. This paper proposes a novel model called CLASSIC. The key novelty is a contrastive continual learning method that enables both knowledge transfer across tasks and knowledge distillation from old tasks to the new task, which eliminates the need for task ids in testing. Experimental results show the high effectiveness of CLASSIC.

==> rebuttal.tex <==

Review #1
What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

This paper presents a novel method called CLASSIC to adapt aspect sentiment models to new domains through contrastive continual learning.
Strengths:

The paper is well written in presenting the method and experiments.
The method is novel and effective and the experiments are extensive on many baselines.
Weakness:

The paper did not address the challenge of aspect vs. document sentiment analysis for domain incremental learning.
Is CLASSIC is able to outperform the previous models on the document sentiment task as well?
Reasons to accept

The first attempt to focus on aspect sentiment classification (ASC) in the domain incremental learning (DIL) setting, though there are previous attempts to work on document sentiment classification in the DIL setting
The paper proposes a novel method called CLASSIC to adapt BERT into ASC continual learning, which allows models to adapt to any seen domain without knowing the task id in testing.
This paper conducts extensive experiments on 46 baseline methods and shows their proposed method is effective and outperforms all the baselines.
Reasons to reject

one minor point. the paper has not discussed the proposed method with previous approaches for document sentiment classification. To adapt previous models to the ASC can potentially be unfair to the previous models.
Reproducibility:	5
Overall Recommendation - Long Paper:	3.5




Review #2
What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

This paper proposes a contrastive continual model for aspect sentiment classification tasks on domain incremental learning scenario. Authors try to give the aspect sentiment classification result when cannot access to task/domain type. To tackle this problem, authors combines previous trained representation via Contrastive Ensemble Distillation. Additionally, to share the knowledge in current task view and previous task's views, author proposes Knowledge Sharing Loss for back of the information. Model outperforms 46 baselines on the sequences of 19 ASC tasks.
Strengths:

This paper proposes domain incremental learning setting in aspect sentiment classification.

This paper proposes a contrastive continual model for this setting and outperform continual learning baselines.

Weaknesses:

The proposed model has weak relationship with aspect sentiment classification task, and can be applied to many domain incremental classification settings.

The contrastive learning objectives in model are bit trivial and the relation between CED and CKS is vague.

The experiment and analysis of this paper is insufficient, and the conducted experiments cannot tell the function of each subsystem in model.

Reasons to accept

This paper proposes domain incremental learning setting in aspect sentiment classification, which is very common in industry applications.
The proposed model outperform non-continual learning and continual learning models on the sequence off 19 ASC tasks.

Reasons to reject

Though the scenario is common in application of ASC systems, their proposed model has weak relationship with ASC, and can be applied to SA or other domain incremental classification settings.
The contrastive learning objectives in model are bit trivial. The relation between CED object and CKS object is vague and overlapped during parameter optimization.

The experiment and analysis of this paper is insufficient, authors many conduct main experiment and ablation. The result in Table 3 cannot give clear information to figure out the function of each part of model.

Questions for the Author(s)

What is the motivation of using CSC? Can you give some explanations about why CSC is useful in CLASSIC? The improvement of using contrastive supervised learning in you model is obvious. But what is you motivation of it, or just a trick for better result? The results in Table2 show the CSC has different effect on baselines. And can you explain why CSC is good for CLASSIC.

The CKS and CED objective seems overlapped. Can you give experimental support on how these two objective effect?

The dataset of the continual learning is unbalanced. SemEval-2014 takes more then half part of datasets. So, can you provide Acc and MF1 on every tasks for better understanding?

4-1. Equation 6 is strange from my understanding. Why the index of positive sample pair is 2n-1 and 2n? In this case, you need 4N samples in single batch, which is conflict to the definition in Sec 3.1.

4-2. Why you use teacher's negative pairing in Equation 6? In common contrastive distillation, the negative pairs are Teacher_i(n) and Student(j).

Missing References

Ke, Zixuan, Hu Xu, and Bing Liu. "Adapting BERT for Continual Learning of a Sequence of Aspect Sentiment Classification Tasks"
Your paper has a lot of similar concepts with above one, and may be misappropriate without citing this paper.

Typos, Grammar, Style, and Presentation Improvements

If you can give clear explanation of 4-1, 4-2, I suggest you to modify the paper for easy accessing.
Reproducibility:	5
Overall Recommendation - Long Paper:	2.5





Review #3
What is this paper about, what contributions does it make, and what are the main strengths and weaknesses?

This paper deals with the problem of Aspect Sentiment Classification (ASC). The proposed approach is able to deal with a sequence of ASC tasks without knowing the task ids in testing. For doing that, contrastive continual learning is used. The main contributions of the paper are the the use of domain incremental learning for solving a sequence of ASC problems and the specific model they propose: CLASSIC.
The strengths of the paper are: On the one hand, the novelty of the approach that authors propose, that is the combination of different deep learning methods employed to solve a complicated problem, like the one presented. On the other hand, the paper is well written and easy to follow. The structure makes it easy to understand the work. A good review of the related work is carried out in Section 2 that helps to understand which is the work's starting point. The experimental setup is also a plus, given the extensive comparison work with very diverse approaches.

The weakness of the paper might be the specificity of the work, that makes it a bit difficult to find usefulness in other domains and the obtained improvements that are not so significant in some cases.

Reasons to accept

I think that it is a very interesting approach in a new framework. It considers continual learning that nowadays is a very important approach considering the ethical issues related to data, that are more and more present in research. Contrastive learning is also important to solve the problems of scarcity of data. These approaches are used in a novel way to solve a complex ASC problem.
Reasons to reject

The only risk I can think of is that it is difficult to directly extend the approach to other similar problems and that the improvements achieved with the proposed model might not be statistically signifcant.
Questions for the Author(s)

Did you think about running a statistical significance test? At least for the most similar results?
The presented work seems to be somehow inspired by the work described in (Sun et al., 2020) and also the results are similar. I can see that LAMOL is not devoted to this specific problem. But could you briefly provide the main difference of the two approaches in the related work. I think that it would enrich the paper.

Did you think on which other NLP problmes might be improved using similar approaches?

Typos, Grammar, Style, and Presentation Improvements

line 84-85 contrative -> contrastive
Reproducibility:	5
Overall Recommendation - Long Paper:	4


Anawer: 

https://docs.google.com/document/d/1XtWDS45TvaGmexb1WamLudqzIQzv7rBd--xoDFJcJJQ/edit?usp=sharing


